Improving Graduation Rate Estimates Using Regularly Updating Multi-Level Absorbing Markov Chains

American universities use a procedure based on a rolling six-year graduation rate to calculate statistics regarding their students' final educational outcomes (graduating or not graduating). As~an alternative to the six-year graduation rate method, many studies have applied absorbing Markov chains for estimating graduation rates. In both cases, a frequentist approach is used. For~the standard six-year graduation rate method, the frequentist approach corresponds to counting the number of students who finished their program within six years and dividing by the number of students who entered that year. In the case of absorbing Markov chains, the frequentist approach is used to compute the underlying transition matrix, which is then used to estimate the graduation rate. In this paper, we apply a sensitivity analysis to compare the performance of the standard six-year graduation rate method with that of absorbing Markov chains. Through the analysis, we highlight significant limitations with regards to the estimation accuracy of both approaches when applied to small sample sizes or cohorts at a university. Additionally, we note that the Absorbing Markov chain method introduces a significant bias, which leads to an underestimation of the true graduation rate. To~overcome both these challenges, we propose and evaluate the use of a regularly updating multi-level absorbing Markov chain (RUML-AMC) in which the transition matrix is updated year to year. We empirically demonstrate that the proposed RUML-AMC approach nearly eliminates estimation bias while reducing the estimation variation by more than 40%, especially for populations with small sample sizes.

==> background.tex <==
%\section{Literature Review}

 %Machine learning and data mining tools have recently gained popularity in predicting students academic performance, mainly due to the large size and dimension of the educational data sets. Educational data mining refers to the application of machine learning, statistic and data mining in the field of education. Research in educational data mining are mostly concerned with predicting student performance, identifying at-risk students and determining factors that affect students' outcome \cite{agnihotri2014building,ayan2008prediction,bridgeman2008predicting,choi2018learning,huang2013predicting}. Marbouti, Diefes-Duxb, and Madhavanb \cite{marbouti2016models} applied different machine learning algorithms such as support vector machine, K-nearest neighbors, and naive Bayes classifier to predict students' course grades. The results show that variables such as mid-term and homework grades and in class quizzes are the most important factors in predicting final grades.

%Fike \cite{fike2008predictors} investigated factors that affects fall-to-spring and fall-to-fall retention for 9200 first-time-students. The results of his study show that parameters such as internet-based courses, financial aid, credits enrolled in the first fall semester, and parents education level have significant impact on student's persistence. Soria and Stebleton \cite{soria2012first} compared retention and academic engagement (combining academic participation and identification) for both first-generation and non-first-generation students. First-generation students are those which are first in their family to pursue a bachelor's degree. The results show that first-generation students are more likely to leave school before graduation.  They also are expected to show less academic engagement compared to the non first generation students.

%Nakajima, Dembo and Mossler \cite{nakajima2012student} studied the impact of demographic, academic, financial, and psychosocial variables on students' retention rate and student persistence in colleges. Results indicate that financial aid, work hours, age, and cumulative GPA are the most important factors influencing student persistence; among which cumulative GPA shows the strongest impact. 









==> data.tex <==
\section{Student Data description} 
To compute the transition probabilities in our baseline Markov model, we use students' data records collected from \censor{UCF}, a large public universities in the United States. The data set consists of demographic information as well as admission type, degree awarded and graduation status for about 17000 undergraduate students between the years of 2008 and 2017. Our data set includes both FTIC and transfer students; however, to meet the federal definition of a program graduation rate, we only consider FTIC students for the purpose of this study.\\
Each Student is distinguished by a unique identifier that helps us to track students flow between absorbing Markov chain states (students academic levels) that are illustrated in Figure \ref{fig:Transition_flow}.




